A pulsed, mono-energetic and angular-selective UV photo-electron source for the commissioning of the KATRIN experiment

The KATRIN experiment aims to determine the neutrino mass scale with a sensitivity of 200 meV/c^2 (90% C.L.) by a precision measurement of the shape of the tritium $\beta$-spectrum in the endpoint region. The energy analysis of the decay electrons is achieved by a MAC-E filter spectrometer. To determine the transmission properties of the KATRIN main spectrometer, a mono-energetic and angular-selective electron source has been developed. In preparation for the second commissioning phase of the main spectrometer, a measurement phase was carried out at the KATRIN monitor spectrometer where the device was operated in a MAC-E filter setup for testing. The results of these measurements are compared with simulations using the particle-tracking software "Kassiopeia", which was developed in the KATRIN collaboration over recent years.

==> definitions.tex <==
\RequirePackage{ifxetex}

% Custom math symbols
\ifxetex
    \renewcommand{\vec}[1]{\rightharpoonaccent{#1}}
\else
    %\newcommand{\tightoverset}[2]{\mathop{#2}\limits^{\vbox to -.5ex{\kern-0.8ex\hbox{$#1$}\vss}}}
    %\renewcommand{\vec}[1]{\tightoverset{\rightharpoonup}{#1}}
\fi
%\renewcommand{\epsilon}{\varepsilon}
%\renewcommand{\phi}{\varphi}
%\renewcommand{\theta}{\vartheta}
\newcommand{\eps}{\epsilon}

\DeclareMathOperator\const{const.}
\DeclareMathOperator\cov{cov}
\DeclareMathOperator\erf{erf}
\DeclareMathOperator\sign{sgn}
\DeclareMathOperator\normal{norm}
\DeclareMathOperator\poisson{poiss}
\DeclareMathOperator\uniform{uni}
\DeclareMathOperator\imag{i}

% Custom math commands
%\newcommand{\dx}[2][]{\mathrm{d}^{#1}{#2}}%                                     \dx{x} -> dx
\newcommand{\dx}[1]{\mathrm{d}{#1}}%                                            \dx{x} -> dx
\newcommand{\ddx}[1]{\mathrm{d}^2{#1}}%                                         \ddx{x} -> d²x
\newcommand{\dddx}[1]{\mathrm{d}^3{#1}}%                                        \dddx{x} -> d³x
\newcommand{\diff}[2]{\dfrac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}%                  \diff{f}{x} -> df/dx
\newcommand{\ddiff}[3]{\dfrac{\mathrm{d}{#1}^2}{\mathrm{d}{#2}\mathrm{d}{#3}}}% \ddiff{f}{x}{y} -> df²/dxdy
\newcommand{\partdiff}[2]{\dfrac{\partial{#1}}{\partial{#2}}}%                  \partdiff{f}{x} -> df/dx
\newcommand{\starred}[1]{{#1}^{\star}}%                                         \starred{x} -> x*
\newcommand{\smalltext}[1]{\text{\footnotesize{#1}}}
\newcommand{\mtext}[1]{\quad\text{#1}\;\;}
\newcommand{\mbreak}{\\[2ex]}

% Custom text commands
\newcommand{\ie}{\mbox{i.\,e.}}
\newcommand{\eg}{\mbox{e.\,g.}}
\newcommand{\wrt}{\mbox{w.\,r.\,t.}}
\newcommand{\etc}{\mbox{etc.}}

% Custom highlighting commands
\newcommand{\caps}[1]{\textsc{#1}}
\newcommand{\strong}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\abbrev}[3]{#1{#2} (#3)\nomenclature{#3}{#2}}
\newcommand{\abbrevs}[3]{#1{#2s} (#3s)\nomenclature{#3}{#2}}
\newcommand{\bfitem}[1]{\item\textbf{#1:}}

% Custom marker commands
\newcommand{\fixme}[1]{\todo[inline,color=red!60]{FIXME: #1}}
\newcommand{\missingref}[1]{\todo[inline,color=green!60]{REF: #1}}
\newcommand{\explain}[1]{\todo[inline,color=yellow!80]{#1}}

% Abbreviations: Mathematics
\newcommand{\onehalf}{\texorpdfstring{\ensuremath{\frac{1}{2}}}{1/2}}
\newcommand{\onethird}{\texorpdfstring{\ensuremath{\frac{1}{3}}}{1/3}}
\newcommand{\bigO}[1]{\ensuremath{\mathcal{O}(#1)}}%                            \bigO{x} -> O(x)

% Abbreviations: Nuclear physics
\newcommand{\isotope}[2]{\texorpdfstring{\ensuremath{{}^{\text{#2}}\text{#1}}}{#1-#2}}
\newcommand{\Rn}[1]{\isotope{Rn}{#1}}
\newcommand{\Po}[1]{\isotope{Po}{#1}}
\newcommand{\Kr}[1]{\isotope{Kr}{#1}}
\newcommand{\Rb}[1]{\isotope{Rb}{#1}}
\newcommand{\Pb}[1]{\isotope{Pb}{#1}}

% Abbreviations: Particle physics
\newcommand{\neutrino}{\ensuremath{\Pneutrino}}
\newcommand{\antineutrino}{\ensuremath{\APneutrino}}
\newcommand{\anyneutrino}{\ensuremath{\Pnu}}
\newcommand{\electron}{\ensuremath{\Pelectron}}
\newcommand{\positron}{\ensuremath{\Ppositron}}
\newcommand{\muon}{\ensuremath{\Pmuon}}
\newcommand{\tauon}{\ensuremath{\Ptauon}}
\newcommand{\antimuon}{\ensuremath{\APmuon}}
\newcommand{\antitauon}{\ensuremath{\APtauon}}
\newcommand{\uquark}{\ensuremath{\Pup}}
\newcommand{\dquark}{\ensuremath{\Pdown}}
\newcommand{\cquark}{\ensuremath{\Pcharm}}
\newcommand{\squark}{\ensuremath{\Pstrange}}
\newcommand{\tquark}{\ensuremath{\Ptop}}
\newcommand{\bquark}{\ensuremath{\Pbottom}}
\newcommand{\uquarkbar}{\ensuremath{\APup}}
\newcommand{\dquarkbar}{\ensuremath{\APdown}}
\newcommand{\cquarkbar}{\ensuremath{\APcharm}}
\newcommand{\squarkbar}{\ensuremath{\APstrange}}
\newcommand{\tquarkbar}{\ensuremath{\APtop}}
\newcommand{\bquarkbar}{\ensuremath{\APbottom}}
\newcommand{\proton}{\ensuremath{\Pproton}}
\newcommand{\neutron}{\ensuremath{\Pneutron}}
\newcommand{\deuteron}{\ensuremath{\Pdown}}
\newcommand{\betabeta}[1]{\ensuremath{{#1}\neutrino\beta\beta}}

% Abbreviations: Technical
\newcommand{\CL}[1]{{#1}\%~\mbox{C.\,L.}}
\newcommand{\LN}[1]{\texorpdfstring{\ensuremath{\mathrm{LN}_{2}}}{LN2}}
\newcommand{\ExB}{\ensuremath{E \times B}}
\newcommand{\chisqndf}{\ensuremath{\chi^2 / \mathrm{ndf}}}
\newcommand{\syst}[1]{\ensuremath{#1\mathrm{(sys)}}}
\newcommand{\stat}[1]{\ensuremath{#1\mathrm{(stat)}}}
%\newcommand{\SIerr}[4]{\SI[parse-numbers=false]{( #1 \pm \syst{#2} \pm \stat{#3} )}{#4}}
\newcommand{\SIerr}[4]{\ensuremath{\SI{#1}{#4} \pm \syst{\SI{#2}{#4}} \pm \stat{\SI{#3}{#4}}}}
%\newcommand{\start}{\ensuremath{\mathrm{start}}}
%\newcommand{\mag}{\ensuremath{\mathrm{mag}}}
%\newcommand{\max}{\ensuremath{\mathrm{max}}}
\newcommand{\longit}[2][]{\ensuremath{{#2}^{\mathrm{#1}}_{\parallel}}}
\newcommand{\transv}[2][]{\ensuremath{{#2}^{\mathrm{#1}}_{\perp}}}
\newcommand{\magnit}[2][]{\ensuremath{|\vec{#2}^{\mathrm{#1}}|}}

\newcommand{\WWU}{WWU~M{\"u}nster}
\newcommand{\KIT}{KIT~Karlsruhe}

\newcommand{\figcaption}[2]{\caption[#1]{{#1} {#2}}}
\newcommand{\runlist}[1]{\hspace*{\fill}\mbox{\fontfamily{\sfdefault}\selectfont\footnotesize Runs:~#1}}

\newcommand{\appendixpdf}[4][]{\includepdf[pages=-,pagecommand=\section*{#3}{\small #4},scale=.8,offset=0mm -25mm,#1]{#2}}
\newcommand{\appendixcode}[4][]{\newpage\section*{#3}{\small #4}\lstinputlisting[#1]{#2}}


% Hyphenation patterns
\hyphenation{%
analy-sis
an-a-lyz-ing
lon-gi-tu-di-nal
trans-ver-sal
spec-tro-me-ter
mag-net-ic
meth-od
elec-tron-an-ti-neu-tri-no
pho-to-elec-tron
pho-to-emis-sion
mi-cro-wave
back-ground
lmfit
minuit
migrad
simplex
minos
emcee
}

